From Holant To #CSP And Back: Dichotomy For Holant$^c$ Problems

We explore the intricate interdependent relationship among counting problems, considered from three frameworks for such problems: Holant Problems, counting CSP and weighted H-colorings. We consider these problems for general complex valued functions that take boolean inputs. We show that results from one framework can be used to derive results in another, and this happens in both directions. Holographic reductions discover an underlying unity, which is only revealed when these counting problems are investigated in the complex domain $\mathbb{C}$. We prove three complexity dichotomy theorems, leading to a general theorem for Holant$^c$ problems. This is the natural class of Holant problems where one can assign constants 0 or 1. More specifically, given any signature grid on $G=(V,E)$ over a set ${\mathscr F}$ of symmetric functions, we completely classify the complexity to be in P or #P-hard, according to ${\mathscr F}$, of \[\sum_{\sigma: E \rightarrow \{0,1\}} \prod_{v\in V} f_v(\sigma\mid_{E(v)}),\] where $f_v \in {\mathscr F} \cup \{{\bf 0}, {\bf 1}\}$ ({\bf 0}, {\bf 1} are the unary constant 0, 1 functions). Not only is holographic reduction the main tool, but also the final dichotomy can be only naturally stated in the language of holographic transformations. The proof goes through another dichotomy theorem on boolean complex weighted #CSP.

==> Background.tex <==
\section{Definitions and Background}
\begin{theorem}\label{thm-holant-star}
Let $\mathscr{F}$ be a set of symmetric signatures over $\mathbb{C}$.
Then $\rm{Holant}^*(\mathscr{F})$ is computable in polynomial time
in the following three cases. In all other cases,
$\rm{Holant}^*(\mathscr{F})$ is \#P-hard.
\begin{enumerate}
	\item Every signature in $\mathscr{F}$ is of arity no more than two;
	\item There exist two constants $a$ and $b$ (not both zero, depending
		only on $\mathscr{F}$), such that for all signatures
		$[x_0,x_1,\ldots,x_k] \in \mathscr{F}$ one of the two conditions is
		satisfied: (1) for every $k=0,1,\ldots,n-2$, we have
		$ax_{k}+bx_{k+1}-ax_{k+2}=0$; (2) $n=2$ and the signature
		$[x_0,x_1,x_2]$ is of form $[2a\lambda,b\lambda,-2a\lambda]$.
	\item For every signature $[x_0,x_1,\ldots,x_n] \in \mathscr{F}$, one
		of the two conditions is satisfied: (1) For every $k=0,1,\ldots,n-2$,
		we have $x_{k}+x_{k+2}=0$; (2) $n=2$ and the signature $[x_0,x_1,x_2]$
		is of form $[\lambda,0,\lambda]$.
\end{enumerate}
\end{theorem}
\begin{definition}\label{def-mathcal-f}
\begin{eqnarray*}
	\mathscr{F}_1 & = &
		\{\lambda([1,0]^{\otimes k}+i^r[0,1]^{\otimes k}) |
			\lambda \in \mathbb{C}, k=1,2, \ldots, r=0,1,2,3\}; \\
	\mathscr{F}_2 & = &
		\{\lambda([1,1]^{\otimes k}+i^r[1,-1]^{\otimes k}) |
			\lambda \in \mathbb{C}, k=1,2, \ldots, r=0,1,2,3\}; \\
	\mathscr{F}_3 & = &
		\{\lambda([1,i]^{\otimes k}+i^r[1,-i]^{\otimes k}) |
			\lambda \in \mathbb{C}, k=1,2, \ldots, r=0,1,2,3\}; \\
	\mathscr{F} & = & \mathscr{F}_1 \cup \mathscr{F}_2 \cup
		\mathscr{F}_3
\end{eqnarray*}
\end{definition}
\begin{theorem}\label{thm-base-holant-c}
Let $\mathscr{G}$ be a set of real symmetric signatures. Then
$\rm{Holant}^c(\mathscr{G})$ is computable in polynomial time if
(1) $\rm{Holant}^*(\mathscr{G})$ is computable in polynomial time, or
(2) $\mathscr{G} \subseteq \mathscr{F}$. Otherwise, $\rm{Holant}^c(\mathscr{G})$
is \#P-hard.
\end{theorem}

\begin{definition}
We now define several classes of transformations.
Let $\omega=e^{2 \pi i/3}$.
\begin{displaymath}
\mathscr{T}_0 \triangleq \left\{
	\left[
		\begin{array}{c c}
			1 & 0 \\
			0 & 1
		\end{array}
	\right],
	\left[
		\begin{array}{c c}
			\frac{1}{\sqrt{\omega}} & 0 \\
			0 & \sqrt{\omega}
		\end{array}
	\right],
	\left[
		\begin{array}{c c}
			\frac{1}{\omega} & 0 \\
			0 & \omega
		\end{array}
	\right]
	\right\}
\end{displaymath}
\begin{displaymath}
\mathscr{T}_f \triangleq \{T \mid
	[1,0,1]T^{\otimes 2}, [1,0]T, [0,1]T \in \mathscr{F}\}
\end{displaymath}
\begin{displaymath}
\mathscr{T} \triangleq \{ T_0T \mid
	T_0 \in \mathscr{T}_0, T \in \mathscr{T}_f\}
\end{displaymath}
\end{definition}
\begin{definition}
A $k$-ary function $f(x_1,\ldots,x_k)$ is affine if it
has the form
\begin{displaymath}
\chi_{AX=0}i^{\sum_{i=1}^{n}\langle \alpha_i,X\rangle}
\end{displaymath}
where $X=(x_1,x_2,\ldots,x_k,1)$, and $\chi$ is an indicator function
such that $\chi_{AX=0}$ is 1 iff $AX=0$. Note that the inner
product is calculated over $\mathbb{F}_2$, while the
total summation is over $\mathbb{F}_4$. We use $\mathscr{A}$
to denote the set of all affine functions.

We use $\mathscr{P}$
to denote the set of functions which can be expressed as a
product of unary functions, binary equality functions ($[1,0,1]$)
and binary disequality functions ($[0,1,0]$).
\end{definition}
\begin{lemma}\label{lemma-csp-binary}
All tractable functions $[a,b,c]$ from $\mathscr{A} \cup \mathscr{P}$
have one of the following forms: $[x,0,y]$, $[0,x,0]$, $[x^2,xy,y^2]$,
$x[1,\pm i,1]$ or $x[1,\pm 1,-1]$.
\end{lemma}
We use $=_k$ to denote the equality function of arity $k$.
Observe that
\begin{displaymath}
\#\rm{CSP}(\mathscr{F}) \equiv_{\rm T}
	\rm{Holant}\left(\mathscr{F} \cup
		\bigcup_{j=3}^{m}\{=_j\}\right)
\end{displaymath}
Now we paraphrase Theorem 2.1 from \cite{cw-csp}.
\begin{theorem}\label{lemma-csp}
Suppose $\mathscr{F}$ is a set of complex signatures.
If $\mathscr{F} \subseteq \mathscr{A}$ or
$\mathscr{F} \subseteq \mathscr{P}$,
$\rm{Holant}(\mathscr{F}\cup\bigcup_{j=3}^{m}\{=_j\})$
is computable in polynomial time. Otherwise, it is \#P-hard.
\end{theorem}
\begin{definition}
Let $\mathscr{B}_1$, $\mathscr{B}_2$, $\mathscr{U}_1$,
$\mathscr{U}_2$, $\mathscr{D}$ be classes of signatures
defined as follows
\begin{eqnarray*}
	\mathscr{D} & = & \{[x_0,x_1,\ldots,x_k] |
		x_0,x_k \in \mathbb{C} \setminus \{0\},
		x_j=0, \rm{ for all } 1 \leq j \leq k-1\} \\
	\mathscr{B}_1 & = & \{[a,0,b] | a,b \in \mathbb{C}\}
		\cup \{[0,a,0] | a \in \mathbb{C}\} \cup
		\{[x^2,xy,y^2] | x,y \in \mathbb{C}\}\\
	\mathscr{B}_2 & = & \{\lambda[1,0,\pm 1],\lambda[1,0,\pm i]
			| \lambda \in \mathbb{C}\}
		\cup \{[0,a,0] | a \in \mathbb{C}\}	\\
		& & \cup \{\lambda[1,\pm i,1], \lambda[1,\pm 1,1]|
			\lambda \in \mathbb{C}\}
			\cup \{[x^2,xy,y^2] | x,y \in \mathbb{C}\}
\end{eqnarray*}
Let $\mathscr{U}_1$ be the set of all unary signatures and
all degenerate symmetric signatures, and $\mathscr{U}_2$ be a set
of unary or degenerate signatures defined as follows:
\begin{displaymath}
	\mathscr{U}_2 = \{\lambda[1,0]^{\otimes k},
		\lambda[0,1]^{\otimes k}, \lambda[1,\pm 1]^{\otimes k},
		\lambda[1, \pm i]^{\otimes k} | \lambda \in \mathbb{C},
		k \in \mathbb{N}\}
\end{displaymath}
Note that $\mathscr{U}_2 \subseteq \mathscr{U}_1$.
\end{definition}

\begin{definition}
something about interpolation
\end{definition}


==> conclusion.tex <==
\section{Conclusion and Discussion}

==> degenerate.tex <==
\section{Some Special Signatures}
We now
prove a dichotomy result for a special class of signatures:
signatures from $\mathscr{D} \cup \mathscr{U}_1$.

%% lemma 1,0,0,0,alpha 0,1,a
\begin{lemma}\label{lemma01a}
Assume that $a \neq 0$ and $\alpha$ is a root of unity.
Then $\textrm{Holant}([1,0,0,0,\alpha],[0,1,a])$ is \#P-hard.
Similarly, we could show that $\textrm{Holant}([1,0,0,0,\alpha],[a,1,0])$
is also \#P-hard.
\end{lemma}
\begin{proof}
Suppose $\alpha$ is a $r$-th root of unity. Then we can connect $r$
$[1,0,0,0,\alpha]$ together to obtain an equality gadget of arity 4,
and thus all equality gadgets of even arity. With these equality
gadgets, we could realize $[0,1,a^{k}]$ for any $k \in \mathbb{N}$.

The $\textrm{Holant}([1,0,0,0,1]|[0,1,1])$ problem is exactly the
\#4-Regular-Vertex-Cover problem, which is known to be \#P-hard\cite{greenhill}.
If $a$ is a root of unity, then we can realize $[0,1,1]$, which implies that it is
\#P-hard.
Otherwise, we can realize all $[0,1,x]$ by polynomial interpolation. In
particular, we can realize $[0,1,1]$, and thus it is still \#P-hard.

This completes the proof for $\textrm{Holant}([1,0,0,0,\alpha],[0,1,a])$.
The proof for $\textrm{Holant}([1,0,0,0,\alpha],[a,1,0])$ is just
symmetric.
\end{proof}

%% lemma a,1,b 1,0,0,0,1
\begin{lemma}\label{lemmaquada1b}
For non-degenerate complex binary signature $[a,1,b]$, the
instance $\textrm{Holant}^c([a,1,b],[1,0,0,0,1])$ is \#P-hard
unless $a$ and $b$ is one of the following cases:
\begin{enumerate}
	\item $ab=1$
	\item $a=b=0$
	\item $ab=-1$ and $a^{4}=1$. Further, in this case,
		$\textrm{Holant}^c([a,1,b],[1,0,0,0,1])$ has
		the same complexity as
		$\#\textrm{CSP}([a,1,b])$.
\end{enumerate}
\end{lemma}
\begin{proof}
It is obvious that the first two cases are tractable.
Assume now that $a$ and $b$ are not of these cases.
Further, from Lemma \ref{lemma01a}, both $a$ and $b$
must be nonzero.

We can construct $[1,b]$ and $[a,1]$ with $[a,1,b]$,
$[0,1]$ and $[1,0]$. Together with $[1,0,0,0,1]$,
we could obtain $[a^2,0,1]$ and $[1,0,b^2]$.
If either $a$ or $b$ is not a root of unity, then
we could use $[a^2,0,1]$ or $[1,0,b^2]$, and $[a,1]$ or $[b,1]$
to interpolate all unary signatures.
By Theorem \ref{thm-holant-star}, $\textrm{Holant}^*([1,0,0,0,1],[a,1,b])$
is \#P-hard, and therefore so is $\textrm{Holant}^c([1,0,0,0,1],[a,1,b])$.

If, on the other hand, $a$ and $b$ are both root of
unity, then we could obtain $[a,0,0,1]$ and $[1,0,0,b]$ by connecting
$[a,1]$ and $[1,b]$ with $[1,0,0,0,1]$.
We could then connect several copies of these gadgets to obtain
$[1,0,0,1]$, and therefore
equality signature of any arity. This implies that
$\textrm{Holant}^c([a,1,b],[1,0,0,0,1])$ has the same
time complexity as $\#\textrm{CSP}([a,1,b])$.
Thus, according to result of \#CSP,
we have that $ab=-1$ and $a^{4}=1$.
The tractability of this case follows from the result
of Theorem \ref{thm-base-holant-c} and the fact that
$[a,1,b], [1,0,0,0,1] \in \mathscr{F}$.
\end{proof}

%% lemma 1,0,0,0,alpha y0,y1,y2
\begin{lemma}\label{lemma1000a}
Let $\mathscr{Y} \subseteq (\mathscr{B}_1 \cup \mathscr{B}_2 \cup \mathscr{U}_1)$
be a set of symmetric signatures.
Then $\textrm{Holant}^c(\{[1,0,0,0,\alpha]\}\cup\mathscr{Y})$ is \#P-hard
unless
\begin{enumerate}
	\item $\mathscr{Y} \subseteq \mathscr{B}_1 \cup \mathscr{U}_1$
	\item $\mathscr{Y} \subseteq \mathscr{B}_2 \cup \mathscr{U}_2$
		and $\alpha^4=1$
\end{enumerate}
\end{lemma}
\begin{proof}
It is easy to see that when
$\mathscr{Y} \subseteq \mathscr{B}_1 \cup \mathscr{U}_1$,
$\textrm{Holant}^c(\{[1,0,0,0,\alpha]\}\cup\mathscr{Y})$ is always tractable.

Otherwise, it must be the case that there is a binary signature
$[y_0,y_1,y_2] \notin \mathscr{B}_1$, since all unary and degenerate
signatures in $\mathscr{U}_2$ are also contained in $\mathscr{U}_1$.
Consequently, $y_1 \neq 0$. Thus,
we could write it as $[a,1,b]$ after scaling, and both $y_0$
and $y_2$ are non-zero.

Assume that $\alpha$ is not a root of unity. By connecting
two dangling edges of $[1,0,0,0,\alpha]$, we could obtain
signature $[1,0,\alpha]$. Since $y_0$ and $y_2$ are not
both zero, we can get a unary signature $[1,x]$ where
$x \neq 0$. We can use these two signatures to interpolate
all unary signatures. By Theorem \ref{thm-holant-star},
this case is \#P-hard.

If $\alpha$ is a root of unity, then by Lemma \ref{lemma01a},
both $y_0$ and $y_2$ must be nonzero. We could combine
several $[1,0,0,0,\alpha]$ together to get an equality signature
of arity 4. By Lemma \ref{lemmaquada1b} and the fact that
$[y_0,y_1,y_2] \notin \mathscr{B}_1$,
it suffices to consider the tractable cases of
$\#\textrm{CSP}(\mathscr{Y} \cup \{[1,0,0,0,\alpha]\})$,
where $\mathscr{Y} \cap (\mathscr{B}_2 \cup \mathscr{U}_2) \neq \emptyset$.
Therefore, we must have
$\mathscr{Y} \cup \{[1,0,0,0,\alpha]\} \subseteq \mathscr{F}$,
and consequently $\mathscr{Y} \subseteq \mathscr{B}_2 \cup \mathscr{U}_2$,
$\alpha^4=1$.
\end{proof}

We can also show a similar result for $[1,0,0,\alpha]$.
%% lemma 1,0,0,alpha y0,y1,y2
\begin{lemma}\label{lemma100a}
Let $\mathscr{Y} \subseteq (\mathscr{B}_1 \cup \mathscr{B}_2 \cup \mathscr{U}_1)$
be a set of complex symmetric signatures.
Then $\textrm{Holant}^c(\{[1,0,0,\alpha]\}\cup\mathscr{Y})$ is
tractable iff
\begin{enumerate}
	\item $\mathscr{Y} \subseteq \mathscr{B}_1 \cup \mathscr{U}_1$
	\item $\alpha^4=1$ and $\mathscr{Y} \subseteq \mathscr{B}_2
		\cup \mathscr{U}_2$.
\end{enumerate}
\end{lemma}
\begin{proof}
If $\alpha$ is not a root of unity, then we have
\begin{eqnarray*}
	& & \textrm{Holant}^c(\{[1,0,0,\alpha]\}\cup\mathscr{Y}) \\ & \equiv_{\rm T} &
		\textrm{Holant}([1,0,1]|\{[1,0,0,\alpha],[1,0],[0,1]\}\cup\mathscr{Y})
\end{eqnarray*}
$\alpha$ is not a root of unity, so we could interpolate $[1,0,0,1]$ on RHS,
therefore
\begin{eqnarray*}
& &	\textrm{Holant}^c(\{[1,0,0,\alpha]\}\cup\mathscr{Y}) \\
		& \equiv_{\rm T} & \#\textrm{CSP}(\{[1,0,0,\alpha],[1,0],[0,1]\}\cup\mathscr{Y})
\end{eqnarray*}
Since $\alpha$ is not a root of unity, $[1,0,0,\alpha]$ is of product type, so all
signatures in $\mathscr{Y}$ must also be of product type, that is
\begin{displaymath}
\mathscr{Y} \subseteq \mathscr{B}_1 \cup \mathscr{U}_1
\end{displaymath}
\begin{figure}
	\includegraphics[width=\textwidth]{gp4.pdf}
	\caption{We use this gadget to construct $[1,0,0,0,\alpha^{2k}]$ recursively.
		The ternary signatures in this gadget are all $[1,0,0,a]$'s.}
	\label{fig-gp4}
\end{figure}
If $\alpha$ is a root of unity, then we could construct $[1,0,0,0,\alpha^{2k}]$ on RHS
for any $k$ with the gadget in Figure \ref{fig-gp4}, and particularly, we have $[1,0,0,0,1]$
on RHS. Consequently, we have
\begin{eqnarray*}
& & \textrm{Holant}^c(\{[1,0,0,\alpha]\}\cup\mathscr{Y}) \\
& \equiv_{\rm T} & \textrm{Holant}^c(\{[1,0,0,\alpha],[1,0,0,0,1]\}\cup\mathscr{Y})
\end{eqnarray*}
By Lemma \ref{lemma1000a}, either
\begin{displaymath}
(\{[1,0,0,\alpha]\} \cup \mathscr{Y}) \subseteq (\mathscr{B}_1 \cup \mathscr{U}_1)
\end{displaymath}
or
\begin{displaymath}
(\{[1,0,0,\alpha]\} \cup \mathscr{Y}) \subseteq (\mathscr{B}_2 \cup \mathscr{U}_2)
\end{displaymath}
The first condition is equivalent to $\mathscr{Y} \subseteq (\mathscr{B}_1 \cup \mathscr{U}_1)$,
and therefore is obviously tractable. The second condition is equivalent to
$\mathscr{Y} \subseteq (\mathscr{B}_2 \cup \mathscr{U}_2)$ and $\alpha^4=1$, and the
tractability of this case follows from Theorem \ref{thm-base-holant-c}.
\end{proof}

Summing up the above two lemmas, we get the following general result.
%% lemma 1,0,...,0,alpha y0,y1,y2
\begin{lemma}\label{lemmageneraldeg}
Let $X=[1,0,\ldots,0,\alpha]$ be a signature of arity not smaller
than 3, and
$\mathscr{Y} \subseteq (\mathscr{B}_1 \cup \mathscr{B}_2 \cup \mathscr{U}_1)$
a set of complex symmetric signatures. $\textrm{Holant}^c(\{X\}\cup\mathscr{Y})$ is
tractable iff
\begin{enumerate}
	\item $\mathscr{Y} \subseteq \mathscr{B}_1 \cup \mathscr{U}_1$
	\item $\mathscr{Y} \subseteq \mathscr{B}_2 \cup \mathscr{U}_2$ and
		$\alpha^4=1$
\end{enumerate}
\end{lemma}
\begin{proof}
``Only if'':
If the arity of $X$ is odd, we can connect the edges of $X$ to obtain
a ternary signature $[1,0,0,\alpha]$ and use Lemma \ref{lemma100a};
otherwise we could construct $[1,0,0,0,\alpha]$ and use Lemma
\ref{lemma1000a}.

``If'':
The tractability of the first case is easy.
For the second case, observe that all signatures are affine, and thus we
could apply the polynomial time algorithm for \#CSP.
\end{proof}

\begin{lemma}\label{lemma-main-deg}
Let $\mathscr{F} \subseteq (\mathscr{D} \cup \mathscr{U}_1 \cup \mathscr{B}_1 \cup \mathscr{B}_2)$
be a set of complex symmetric signatures with at least one signature
of arity greater than 2.
$\textrm{Holant}^c(\mathscr{F})$ is tractable iff
\begin{enumerate}
	\item All binary signatures are from $\mathscr{B}_1$
	\item For all signatures $[a,0,\ldots,0,b] \in \mathscr{F} \cap
		\mathscr{D}$ of arity greater than 2,
		we have $\frac{b}{a} \in \{\pm 1, \pm i\}$,
		all binary signatures are from $\mathscr{B}_2$,
		and all unary or degenerate signatures from $\mathscr{U}_2$
\end{enumerate}
\end{lemma}
\begin{proof}
If all binary signatures are from $\mathscr{B}_1$, then the tractability
is quite straightforward.

On the other hand, there are some binary signatures $Y \in \mathscr{Y}$
not in $\mathscr{B}_1$. According to Lemma \ref{lemmageneraldeg},
it must be that $\mathscr{Y} \subseteq \mathscr{B}_2 \cup \mathscr{U}_2$
and all $\frac{b}{a}$'s must satisfy $(\frac{b}{a})^4=1$.
We could use the algorithm for \#CSP to solve this instance.
\end{proof} 


==> figures.tex <==
\section{Figures}

\begin{figure}[httb]
	\includegraphics[width=\textwidth]{gp1.pdf}
	\caption{A recursive gadget we used to construct $[1,0,a^{3k+1}]$ on LHS.
			Ternary signatures are $[1,0,0,1]$, and binary signatures are
			$[1,0,a]$.}
	\label{fig-gp1}
\end{figure}

\begin{figure}[httb]
	\centering
	\includegraphics[width=\textwidth]{gp2.pdf}
	\caption{The recursive gadget we used to realize $[1,0,0,-\omega_{3^{(l-1)}}^{mbk_0/2}]$
			where $m$ is an odd integer. All ternary gadgets are
			$[1,0,0,-\omega_{3^{(l-1)}}^{bk_0/2}]$.}
	\label{fig-gp2}
\end{figure}


\begin{figure}[httb]
	\centering
	\includegraphics{gp3.pdf}
	\caption{We use this gadget to realize $[a,0,1]$. The ternary signature is
		$[1,0,0,1]$, the binary signatures are $[0,1,0]$ and the unary one is
		$[1,a]$.}
	\label{fig-gp3}
\end{figure}

\begin{figure}[httb]
	\centering
	\includegraphics{g0.pdf}
	\caption{All signatures are $[v,1,0,0]$.}
	\label{fig-g0}
\end{figure}

\begin{figure}[httb]
	\begin{minipage}[t]{0.55\linewidth}
		\centering
		\includegraphics[width=\textwidth]{gt1.pdf}
		\caption{We use this gadget to construct binary disequality on LHS.
			Ternary signature is $=_3$, binary signature is $[1,\pm i,1]$.}
		\label{fig-gt1}
	\end{minipage}
	\hspace{0.02\linewidth}
	\begin{minipage}[t]{0.4\linewidth}
		\centering
		\includegraphics[width=\textwidth]{gt2.pdf}
		\caption{We use this gadget to construct binary disequality on LHS.
			Ternary signature is $=_3$, binary signature is $[1,\pm 1,-1]$.}
		\label{fig-gt2}
	\end{minipage}
\end{figure}


==> intro2.tex <==
\section{Introduction}
In order to study the complexity of counting problems, several
interesting frameworks have been proposed. One is called counting
Constraint Satisfaction Problems
(\#CSP)~\cite{Bulatov06,Bulatov08,BulatovD03,weightedCSP,FederV98}.
Another well studied framework is called $H$-coloring
or Graph Homomorphism,
 which can be viewed as a special case of
\#CSP
problems~\cite{BulatovG04,BulatovG05,Homomorphisms,DyerGP06,acyclic,DyerG00,DyerG04,GJGT,Hell}.
Recently, we proposed a new refined framework called Holant 
Problems~\cite{FOCS08,STOC09} inspired by Valiant's Holographic 
Algorithms~\cite{HA_FOCS,AA_FOCS}.
One reason such frameworks are interesting is because the language
is {\it expressive} enough so that they can express many natural
counting problems, while {\it  specific} enough so that we can prove
\emph{dichotomy theorems} (i.e., every problem in the class
is either in P or \#P-hard)~\cite{CSPBook}.
By a theorem of Ladner, if P $\not =$ NP, or P $\not =$ \#P,
then such a dichotomy for NP or \#P 
is \emph{false}.
Many natural counting problems can be expressed in all three 
 frameworks. This includes 
counting the number of vertex covers,
the number of $k$-colorings in a graph, and many others. However,
{\it some}
 natural and important counting problems, such as counting the number of
perfect matchings in a graph,  {\it cannot} be expressed as a graph
homomorphism function~\cite{freedman-l-s}, 
but can be naturally expressed as a Holant Problem.
Both \#CSP and Graph Homomorphisms can be viewed as 
special cases of Holant Problems.
The Holant framework of counting problems makes a finer
complexity classification.
% due to its expressibility. 
A rich mathematical structure is uncovered in the 
Holant framework regarding the
complexity of counting problems, which is sometimes difficult even to state
in \#CSP. This is particularly true when we apply holographic
reductions~\cite{HA_FOCS,AA_FOCS,FOCS08}.
%This is also our main language in this paper.

%This notion is motivated by holographic
%reductions proposed by Valiant~\cite{HA_FOCS,AA_FOCS}. 
We give a brief description of the Holant framework here.
%and a more formal definition is given in
%Section~\ref{sec:background}. 
A {\it signature grid} $\Omega = (G,
{\mathscr F}, \pi)$ is a tuple, where $G=(V,E)$ is a graph, and $\pi$
labels each $v \in V$ with a function $f_v \in {\mathscr F}$. We consider
all edge assignments (in this paper 0-1 assignments).
 An assignment $\sigma$ for every $e\in E$
gives an evaluation $\prod_{v \in  V} f_v(\sigma\mid_{E(v)})$, where
$E(v)$ denotes the incident edges of $v$,
and $\sigma\mid_{E(v)}$ denotes the restriction of $\sigma$  to $E(v)$.
 The  counting problem on the instance  $\Omega$
is to compute
\[{\rm Holant}_\Omega=\sum_{\sigma}
\prod_{v\in V} f_v(\sigma\mid_{E(v)}).\] 
For example, consider the {\sc Perfect
Matching} problem on $G$. This problem corresponds to attaching the
{\sc Exact-One} function at every vertex of $G$, and then consider
all 0-1 edge assignments. In this case, ${\rm Holant}_\Omega$ counts
the number of perfect matchings. If we use the {\sc At-Most-One}
function  at every vertex, then we count all (not necessarily
perfect) matchings.
We use the notation
Holant(${\mathscr F}$) to denote the class of Holant problems where all
functions are given by ${\mathscr F}$.


To see that Holant is a more expressive framework, we show that
every \#CSP problem can be directly 
simulated by a Holant problem. Represent
an instance of a \#CSP problem by  a bipartite graph where LHS are
labeled by variables and RHS are labeled by constraints. Now the
signature grid $\Omega$ on this bipartite graph is as follows: Every
variable node on  LHS is labeled with an {\sc Equality} function, every
constraint node on RHS is labeled with the given constraint function. Then
${\rm Holant}_\Omega$ is exactly the answer to the counting CSP
problem. In effect, the {\sc Equality} function on a node in LHS
forces the incident edges to take the same value; this
effectively reduces to a vertex assignment on LHS as
in \#CSP. 
%It follows that \#CSP problems are precisely the special
%case of Holant problems on bipartite graphs where every node in  LHS
%is attached an {\sc Equality} function.
We can show that \#CSP  is equivalent to
Holant problems where  {\sc Equality} functions 
of  $k$ variables, for arbitrary $k$  (denoted by $=_k$), are 
freely  and implicitly available  as constraints.
%
%However the Holant framework is more refined.
However, there is no obvious way to reverse  the above process.
%by simulating Holant with \#CSP in general.
While \#CSP is the same as  adding all $=_k$ to Holant,
 %(actually 3-way
%{\sc Equality} $=_3$ will do), 
the effect of this is non-trivial.
% adding $=_3$ is non-trivial.
From the lens of holographic transformations, $=_3$ is a full fledged
non-degenerate symmetric function of arity 3.
%Additionally,

Meanwhile,
one can consider new classes of counting problems derived from
the Holant framework, which are
difficult to express as \#CSP problems.
One such class, called Holant$^*$ Problems~\cite{STOC09},
is the class of Holant Problems where all 
unary functions are freely available.  If we allow only
two special unary
functions
%functions $[1,0]$ and $[0,1]$
{\bf 0} and {\bf 1} as freely available, then we obtain
the family of counting problems called
 Holant$^c$ Problems,
which is even more appealing.   This is the class
of all Holant Problems (on boolean variables) where one can 
set any particular edge (variable) to 0 or 1 in an input graph.
 
Previously we  proved a dichotomy theorem for
${\rm Holant}^*(\mathscr{F})$, where $\mathscr{F}$
is any set of complex-valued symmetric functions~\cite{STOC09}.
%Holant$^*$ Problems is studied primarily as a technical bridge
%to other classes of counting problems;
It is used to prove a dichotomy theorem for \#CSP in \cite{STOC09}.
For ${\rm Holant}^c(\mathscr{F})$ we could only
prove a dichotomy theorem for real-valued functions.
In this paper we manage to traverse in the other direction, going from \#CSP
to Holant Problems.
%derivations. 
First we establish a dichotomy theorem
for   a special Holant class.
%Problem involving exactly one
%non-degenerate symmetric signature of arity 3,
Second we prove  a more general dichotomy for bipartite Holant Problems.
Finally by going through  \#CSP,
we prove a dichotomy theorem for complex-valued Holant$^c$ Problems.
Now we describe our results in more
detail.

A symmetric function $f: \{0,1\}^k \rightarrow \mathbb{C}$
will be written as $[f_0,f_1,\ldots,f_k]$, where $f_j$ is the value
of $f$ on inputs of Hamming weight $j$.
%(E.g., the constant unary functions {\bf 0} and {\bf 1} are
%$[1,0]$ and $[0,1]$.)
Our first main result (in
Section \ref{sec-ternary}) is a dichotomy theorem for
%ternary functions. That is a dichotomy theorem
${\rm Holant}(\mathscr{F})$, where
$\mathscr{F}$ contains a single ternary function $[x_0, x_1, x_2, x_3]$.
More generally, as
proved by holographic reductions,
 we get a dichotomy theorem for 
${\rm Holant}([y_0, y_1, y_2] | [x_0, x_1, x_2, x_3] )$
defined on 2-3 regular bipartite graphs. 
Here the notation indicates that every vertex of degree 2
on LHS has label $[y_0, y_1, y_2]$ and every vertex of degree 3
on RHS has label $[x_0, x_1, x_2, x_3]$.
This is the foundation
 of the remaining two dichotomy results in this paper.
Previously we proved a dichotomy theorem 
for  ${\rm Holant}([y_0, y_1, y_2] | [x_0, x_1, x_2, x_3] )$, when
all $x_i$, $y_j$ take values in $\{0,1\}$~\cite{FOCS08}.
Kowalczyk extended this to $\{-1,0,1\}$ in \cite{mike}.
In \cite{TAMC}, we gave a dichotomy theorem for 
${\rm Holant}([y_0, y_1, y_2] | [1,0,0,1] )$, where $y_0, y_1, y_3$
%take arbitrary real numbers. Finally
take arbitrary real values. Finally
this was  extended to arbitrary complex numbers~\cite{cai}.
Our result here is built upon these results, especially~\cite{cai}.

Our second result (Section \ref{sec-holant-to-csp})
is a dichotomy theorem, under a mild condition,
%%%%
%%%% JYC
%%%%  I feel the results in sec 4 {sec-holant-to-csp}
%%%%  is never fully stated in generality, except in the generic case.
%%%%  would it be easy to state a clean statement includng the
%%%%  the non-generic case?  it would be nice to just cite
%%%% what we obtain in sec 3, and move on. instead of mostly refer to
%%%% \cite{cai} with Kowalczyk-Cai.
%%%%
for bipartite Holant problems
${\rm Holant}( \mathscr{F}_1
| \mathscr{F}_2)$.
%where $\mathscr{F}_1$ (respectively $\mathscr{F}_2$)
%contains  some non-degenerate function $[y_0,y_1, y_2]$ of arity 2
%(respectively some non-degenerate $[x_0,x_1,x_2,x_3]$ of arity 3).
To prove that, we first use holographic reductions
%To prove that, in a ``generic'' case,  we first use holographic reductions
%%% i think trechnically i should say the above, namely only in 
%%% a ``generic'' case, to go to [1 0 0 1]
%%% but i think i will leave it vague.
 %to transform the problem to ${\rm Holant}(\mathscr{F}'_1
to transform it to ${\rm Holant}(\mathscr{F}'_1
| \mathscr{F}'_2)$, where we transform
some non-degenerate function $[x_0,x_1,x_2,x_3] \in \mathscr{F}_2$ 
%is transformed
to the {\sc Equality} function $(=_3) = [1, 0, 0, 1] \in \mathscr{F}'_2$.
Then we prove that we can ``realize'' the binary {\sc Equality} function
 $(=_2) = [1,0,1]$ in the 
left side and reduce the problem to
$\#{\rm CSP}(\mathscr{F}'_1 \cup \mathscr{F}'_2)$.
This is a new proof approach.
Previously in~\cite{STOC09},
we reduced a \#CSP problem to a Holant problem and obtained results for \#CSP.
Here, we go the opposite way, using
  results for \#CSP to prove dichotomy theorems for Holant problems.
This is made possible
by our complete dichotomy theorem for boolean complex
weighted \#CSP~\cite{STOC09}. We note that proving this over
$\mathbb{C}$ is crucial, as holographic reductions naturally
go beyond $\mathbb{R}$. We also note that
our dichotomy
theorem here does not require the functions
in $\mathscr{F}_1$ or $\mathscr{F}_2$ to be symmetric.
This will be useful in the future.
%So the theorem  will be useful for 
%can have future applications
%in dichotomy theorems for more general Holant problems.

Our third main result, also the initial motivation of this
%%% JYC i cut out the word "whole"
work, is a dichotomy theorem for
symmetric complex Holant$^c$ problems. This improves
our previous result in \cite{STOC09}.
% which gives a dichotomy
%theorem for symmetric real Holant$^c$ problems.
We made a conjecture in \cite{STOC09} that the dichotomy theorem
stated as Theorem~\ref{thm:holnat-c} is also true for
symmetric complex functions. It turns out that
this conjecture is not correct as stated. 
For example, 
Holant$^c([1,0,i,0])$ is tractable (according to our new theorem),
but not included in the tractable cases by the conjecture.
After isolating these new tractable cases
we prove {\it everything else} is \#P-hard.
In general, non-trivial and previously unknown tractable cases are what make
dichotomy theorems particularly interesting, but at the same
time make them more difficult to prove (especially for hardness proofs). 
The proof approach here is also different from
that of \cite{STOC09}. In \cite{STOC09}, the idea is to interpolate all
unary functions and then use the results for Holant$^*$ Problems.
Here we first prove that we can realize some non-degenerate
ternary function, for which we can use the result of our first
dichotomy theorem. Then we use our second dichotomy theorem
to further reduce the problem to \#CSP and obtain a dichotomy theorem.

The study of Holant Problems is strongly influenced by the
development of holographic algorithms and 
%holographic
reductions~\cite{HA_FOCS,AA_FOCS,STOC07,FOCS08}. Indeed,
holographic reduction is a primary technique in the proof of these
dichotomy results, both for the algorithm design part and the hardness proof
part. More than that, 
%as we can see from the results of this paper,
holographic reduction even provides the correct language for the {\it
statements} of
these dichotomies. 
%Without using holographic reductions to
%normalize a given set of functions, it is not easy to even fully describe
Without using holographic reductions, it is not easy to even fully describe
what are the tractable cases in the dichotomy theorem.
Another interesting observation is that by employing
holographic reductions, complex numbers appear naturally
and in an essential way.
% Thus
%our functions ${\mathscr F}$ are complex valued.
Even if one is only interested in integer or real valued
counting problems, in the complex domain $\mathbb{C}$
 the picture becomes whole.
%As Jacques Hadamard said:
%``The shortest path between two truths in the real domain
%passes through the complex domain.'' (Jacques Hadamard)
%%%%%%%%%% JYC: do you like th French one?
%%%``Le plus court chemin entre deux v\'{e}rit\'{e}s dans le domaine
%%%r\'{e}el passe par le domaine complexe.'' ---Jacques Hadamard.
``It has been written that the shortest and best way between two 
truths of the real domain often passes through the imaginary one.'' 
---Jacques Hadamard.



%%%%%%%%%%%%



==> list-of-T.tex <==
\section{List of Matrices in $\mathscr{T}$}
In this section, we explicitly list all the matrices in the family
$$
\mathscr{T} \triangleq \{T \mid
	[1,0,1]T^{\otimes 2}, [1,0]T, [0,1]T \in \mathscr{A}\},
$$
which is defined and used in the statement of Theorem \ref{thm:main}.
Together with Theorem~\ref{thm-holant-star}, this gives an effective  condition
for tractability of ${\rm Holant}^c$ problems by Theorem~\ref{thm:main}.

As noted before, the set of symmetric signatures in  $\mathscr{A}$ is exactly
$\mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$.
We note that $[1,0,1]T^{\otimes 2}$, $[1,0]T$ and $[0,1]T$ are all
symmetric, as is the requirement $T^{-1} \mathscr{F} \subseteq \mathscr{A}$
in Theorem~\ref{thm:main}. Thus we can replace $\mathscr{A}$
by $\mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$
in the expression $\mathscr{T}$ above.
 
It is obvious that the family $\mathscr{T}$ is closed under a scalar
multiplication. Thus we list them up to a scalar multiple.
%After scaling, symmetric binary signatures in $\mathcal{F}$ are:
%%% JYC: check this symbol
After a scalar multiple, symmetric binary signatures in 
$\mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$ are precisely
\[[1, 0, \pm 1], [1, 0, \pm i], [1, \pm 1, -1], [1, \pm i, 1], 
[0,1,0].\]
We note that this set is invariant under reversal, up to a   
scalar multiple.
Also the unary signatures in
$\mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$, up to a 
scalar multiple,
are $[1, \pm 1]$, $[1,\pm i]$, $[1,0]$ and $[0,1]$.

Before we enumerate all the possibilities, 
we make two observations to simplify this process:
\begin{enumerate}
\item If we exchange the two columns of $T$,
the signature $[1,0,1]T^{\otimes 2}$  becomes its reversal,
%remains unchanged,
%%% JYC:
%%%% if you do columns exchange, $[1,0,1]T^{\otimes 2}$ IS changed.
%%% eg try (1, 2 ; 3, 4)
%%%
%%% if you exchange two rows of T , it is unchagbed...
%%%This is because
%\[ [1,0,1]T^{\otimes 2} = ( (1, 0)^{\otimes 2} + (0, 1)^{\otimes 2} )
%T^{\otimes 2} = ( (1, 0)T)^{\otimes 2} + ((0, 1) T)^{\otimes 2}.\]
%%% i am not sure you want col or row. but looks ike you meant col.
%%%
		and the two numbers in $[1,0]T$ are
 interchanged. Similarly the
two numbers in $[0,1]T$ are interchanged.
 The effect of exchanging the two columns of $T$
is the same as replacing $T$ 
by $T \left[
        \begin{array}{c c}
                0 & 1 \\
                1 & 0
        \end{array}
\right]$. On the other hand,
the holographic transformation 
$\left[
        \begin{array}{c c}                
		0 & 1 \\
                1 & 0        
	\end{array}\right]
\mathscr{A}$ amounts exchanging input
values 0 and 1 for functions in $\mathscr{A}$,
and this operation keeps $\mathscr{A}$ invariant.
 Therefore, we only need to consider
		$[1,0]T \in \{[1,\pm 1], [1, 0], [1, i]\}$,
up to a scalar factor,
in order to determine whether there exists a $T \in \mathscr{T}$ such that
                $\mathscr{F} \subseteq T\mathscr{A}$,
as in Theorem~\ref{thm:main}.
%%% JYC. eg if there was another T' making [1,0]T' =[1, -i]
%%% then use another T, exchanging two column, can get to [-i, 1] equiv to
%%% [1, i]. the same T also keeps [1,0,1]T in A. and makes F in T A.
%%%
%%% but for later, when we "normalize" for [1 0 1]T
%%% we still need to keep [1,0]T = [0,1] case around.  I think. (JYC)
\item If we multiply $\left[\begin{array}{c c}1 & 0 \\0 & -1\end{array}\right]$ on the
		right side of $T$, then $[y_0,y_1,y_2] \triangleq [1,0,1]T^{\otimes 2}$ becomes
		$[y_0,-y_1,y_2]$. 
This operation also preserves the set of arity 2 signatures
listed for $\mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$,
up to  a scalar factor.
The same invariance holds for the set of unary signatures
listed for $\mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$.
%%% this is to multiply -1 to the second entry.
The effect of the holographic transformation
$\left[
        \begin{array}{c c}
                1 & 0 \\
                0 & -1   
        \end{array}\right]
\mathscr{A}$ is to transform the original $f$ to $f \cdot (-1)^{\sum_i x_i}$,
and thus it is in $\mathscr{A}$ iff the original $f \in \mathscr{A}$.
%Furthermore this operation does not affect $[1,0]T$ from item 1.
%%% JYC: actually i have a problem with this.
%%%  once you have used item 1 to make $[1,0]T$ as listed.
%%% can you still make this change of T by right multiply (1 0 ; 0, -1)?
%%% wouldn't that affect $[1,0]T$?  eg wouldn't i have to think
%%% about [1,0]T = (1 -i) from the case in item 1. [1,0]T = (1 i) ???
%%%
So we only need to consider $T$'s such that
		$[1,0,1]T^{\otimes 2} \in \{[1,0,\pm 1], [1,0,\pm i],
[1,1,-1], [1,i,1],[0,1,0]\}$,
up to a scalar factor.

Similarly, we could multiply $\left[\begin{array}{c c}1 & 0 \\ 0 & i\end{array}\right]$
on the right side of $T$. Then we only need to investigate
$[1,0,1]T^{\otimes 2}
 \in \{[1,0,1], [1,0,i], [1,i,1],[0,1,0]\}$,
up to a scalar factor.

\end{enumerate}

We now enumerate all $T$'s, such that $[1,0,1]T^{\otimes 2}, [1,0]T, [0,1]T 
\in \mathscr{F}_1 \cup \mathscr{F}_2 \cup \mathscr{F}_3$.
In the following, we let $\alpha=(1+i)/\sqrt{2}=\sqrt{i}$.

%%% JYC
%%% I knew I said someting that we can remove the second one in each
%%% pair of matrices T in each case, where the secon is obtained from
%%% the first by * (-1) on second row.
%%% but now I am not certain we can omit those.
%%% it is true that for the condition {script T} this multiply -1
%%% to second row does not affect [1,0,1]T and [1,0]T and [0,1]T in {script A}
%%% but I am not sure it does not affect the condition 
%%% given F \subseteq T {script A}.
%%% if we replace T by this * (-1) on second row of T, ie (1 0; 0, -1) * T
%%% it is same as preprocessing the given F by replacing each f \in F
%%% with (-1)^{\sum_i x_i} f.  and then check against the old T
%%% to see if we get all f in F are in T {script A}.
%%%

%%% so unless there is an argument, we should restore the second half 
%%% of the T's listed.


%%% I don't see why you need to both \lambda and \gamma below.
%%% one is enough. i think.

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,1]$, $[1,0]T=\lambda[1,1]$, we have
$T=
\left[
	\begin{array}{c c}
		1 & 1 \\
		1 & -1
	\end{array}
\right]
$.
%,
%\left[
%	\begin{array}{c c}
%		1 & 1 \\
%		-1 & 1
%	\end{array}
%\right].
%\end{displaymath}

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,1]$, $[1,0]T=\lambda[1,-1]$, we have
$
T=
\left[
	\begin{array}{c c}
		1 & -1 \\
		1 & 1
	\end{array}
\right]$.
%,
%\left[
%	\begin{array}{c c}
%		1 & -1 \\
%		-1 & -1
%	\end{array}
%\right].
%\end{displaymath}

For $[1,0,1]T^{\otimes 2}=\gamma[1,0,1]$, $[1,0]T=\lambda[1,\pm i]$, there is no solution.

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,1]$, $[1,0]T=\lambda[1,0]$, we have
$
T=
\left[
	\begin{array}{c c}	
		1 & 0 \\
		0 &  1
	\end{array}
\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,i]$, $[1,0]T=\lambda[1,1]$, we have
$T=
\left[
	\begin{array}{c c}
		1 & 1 \\
		\alpha^3 & \alpha
	\end{array}
\right]$.
%,
%\left[
%	\begin{array}{c c}
%		1 & 1 \\
%		-\alpha^3 & -\alpha
%	\end{array}
%\right].
%\end{displaymath}

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,i]$, $[1,0]T=\lambda[1,-1]$, we have
$T=
\left[
	\begin{array}{c c}
		1 & -1 \\
		\alpha^3 & -\alpha
	\end{array}
\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,i]$, $[1,0]T=\lambda[1,i]$, we have
$T=
\left[
	\begin{array}{c c}
		1 & i \\
		\alpha & -\alpha
	\end{array}
\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[1,0,i]$, $[1,0]T=\lambda[1,0]$, we have
$T=
\left[
	\begin{array}{c c}
		1 & 0 \\
		0 & \alpha
	\end{array}
\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[1,i,1]$, $[1,0]T=\lambda[1,1]$, we have
$T=
\left[\begin{array}{c c}
	1 & 1 \\
	-\alpha^3 & \alpha^3
\end{array}\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[1,i,1]$, $[1,0]T=\lambda[1,-1]$, we have
$
T=\left[\begin{array}{c c}
	1 & -1 \\
	\alpha & \alpha
\end{array}\right]$.


If $[1,0,1]T^{\otimes 2}=\gamma[1,i,1]$, $[1,0]T=\lambda[1,i]$, we have
$T=\left[\begin{array}{c c}
	1 & i \\
	0 & \sqrt{2}
\end{array}\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[1,i,1]$, $[1,0]T=\lambda[1,0]$, we have
$T=
\left[\begin{array}{c c}
	\sqrt{2} & 0 \\
	i & 1
\end{array}\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[0,1,0]$, $[1,0]T=\lambda[1,1]$, we have
$T=
\left[\begin{array}{c c}
	1 & 1 \\
	i & -i
\end{array}\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[0,1,0]$, $[1,0]T=\lambda[1,-1]$, we have
$T=
\left[\begin{array}{c c}
	1 & -1 \\
	-i & -i
\end{array}\right]$.

If $[1,0,1]T^{\otimes 2}=\gamma[0,1,0]$, $[1,0]T=\lambda[1,i]$, we have
$T=
\left[\begin{array}{c c}
	1 & i \\
	-i & -1
\end{array}\right]$.

For $[1,0,1]T^{\otimes 2}=\gamma[0,1,0]$, $[1,0]T=\lambda[1,0]$, there is no solution.



